Adversarial Out-domain Examples for Generative Models

Deep generative models are rapidly becoming a common tool for researchers and developers. However, as exhaustively shown for the family of discriminative models, the test-time inference of deep neural networks cannot be fully controlled and erroneous behaviors can be induced by an attacker. In the present work, we show how a malicious user can force a pre-trained generator to reproduce arbitrary data instances by feeding it suitable adversarial inputs. Moreover, we show that these adversarial latent vectors can be shaped so as to be statistically indistinguishable from the set of genuine inputs. The proposed attack technique is evaluated with respect to various GAN images generators using different architectures, training processes and for both conditional and not-conditional setups.

==> arxiv_Adversarial Out-domain Examples for Generative Models/images/Interpolation/interpolation.tex <==
\begin{figure*}[ht]
    \footnotesize
    \centering
    \textbf{a)} In-domain to In-domain\\
    \includegraphics[scale=.20]{images/Interpolation/indomain_li.pdf}
    
    \textbf{b)} In-domain to Out-domain\\
    \includegraphics[scale=.20]{images/Interpolation/outdomain_li.pdf}

    \textbf{c)} Out-domain to Out-domain\\
    \includegraphics[scale=.20]{images/Interpolation/fulloutdomain_li.pdf}
   % \textbf{c)} Out-domain to Out-domain
    %\includegraphics[scale=.27]{images/Interpolation/fulloutdomain_li.pdf}
    \caption{Three examples of linear interpolation between two latent vectors for a \textit{ProGAN} trained on the \textit{CelebA} dataset. The row (a) depicts the interpolation process between two randomly chosen latent vectors. Row (b) depicts interpolation from a randomly chosen latent vector and an out-domain latent vector. Row (c) depicts interpolation between two out-domain latent vectors.}
    \label{progan_linterpolation}
\end{figure*}

==> arxiv_Adversarial Out-domain Examples for Generative Models/tables/ACGAN_ALL.tex <==
\begin{table*}[tp]
\footnotesize
\caption{\small Results for any \textit{ACGAN} generator. Scores are obtained as the average over test-set results for each of the ten classes present in the generator training-set.}
\centering
\begin{tabular}{lr|rr||rr|}
\multicolumn{2}{c}{}
&\multicolumn{2}{|c||}{(a) \textbf{Normal Latent distribution}}
& \multicolumn{2}{c|}{(b) \textbf{Uniform Latent distribution}} \\
\toprule
   Dataset &  $Z$ dim. &  \textbf{Avg MSE}  & \textbf{Test Succ.} &  \textbf{Avg MSE}  & \textbf{Test Succ.}  \\ \midrule
 CIFAR10 &          100 &  0.023457 &          100\% &  0.019615 &  100\%\\
 CIFAR10 &          256 &  0.013144 &          100\% &  0.009547 &          100\%\\
 CIFAR10 &          512 &  0.009075 &          100\% &  0.005944 &           99\%\\ \midrule
    SVHN &          100 &  0.026686 &          100\% &  0.024732 &          100\% \\
    SVHN &          256 &  0.016879 &          100\% &  0.016268 &          100\%\\
    SVHN &          512 &  0.016291 &          100\% &  0.013707 &           99\%\\
\bottomrule
\end{tabular}
\label{acgan_allresulttable}
\end{table*}


==> arxiv_Adversarial Out-domain Examples for Generative Models/tables/DCGAN_ALL.tex <==
\begin{table*}[ht]
\footnotesize
\caption{\small Results concerning the out-domain generation process on the test-set for all the \textit{DCGAN} generators. The column \textbf{Test Succ.} reports the percentage of out-domain latent vectors which successfully passed statistical tests. The column \textit{Avg MSE*} reports the average \textit{MSE} in the case of complete relaxation of the penalty term $\rho$.}
\centering
\begin{tabular}{lr|rrr||rrr|}
\multicolumn{2}{c}{}
&\multicolumn{3}{|c||}{(a) \textbf{Normal Latent distribution}}
& \multicolumn{3}{c|}{(b) \textbf{Uniform Latent distribution}} \\
\toprule
   Dataset &  $Z$ dim. &  \textbf{Avg MSE} & \textbf{Test Succ.} & Avg MSE* &  \textbf{Avg MSE} & \textbf{Test Succ.} & Avg MSE* \\ \midrule
    CIFAR10 &          100 &  0.010646  & 100\% & 0.008881 & 0.012131  & 100\% & 0.009354\\
    CIFAR10 &          256 &  0.005094  & 100\% & 0.003902 &  0.012131  & 100\% & 0.009354\\
    CIFAR10 &          512 &  0.003693  & 100\% & 0.002710 &  0.003603  & 100\% & 0.002826\\ \midrule
       SVHN &          100 &  0.018569  & 100\% & 0.011541 & 0.016730 & 100\% & 0.011359   \\
       SVHN &          256 &  0.011374  & 100\% & 0.006970 &  0.012121 & 100\%  & 0.007213  \\ 
       SVHN &          512 &  0.009474  & 100\% & 0.005314 &  0.008323  & 100\% & 0.005594 \\ \midrule
 C.MNIST &          100 &  0.063097  & 100\% & 0.040453  &  0.059342  & 100\% & 0.037457 \\
 C.MNIST &          256 &  0.052926  & 100\% & 0.029160 &  0.045851  & 100\% & 0.027178\\
 C.MNIST &          512 &  0.043685  & 100\% & 0.025855 &  0.037946 & 99\%  & 0.022415\\
\bottomrule
\end{tabular}
\label{dcgan_allresulttable}
\end{table*}

